Metric Temporal Equilibrium Logic over Timed Traces

In temporal extensions of Answer Set Programming (ASP) based on linear-time, the behavior of dynamic systems is captured by sequences of states. While this representation reflects their relative order, it abstracts away the specific times associated with each state. However, timing constraints are important in many applications like, for instance, when planning and scheduling go hand in hand. We address this by developing a metric extension of linear-time temporal equilibrium logic, in which temporal operators are constrained by intervals over natural numbers. The resulting Metric Equilibrium Logic provides the foundation of an ASP-based approach for specifying qualitative and quantitative dynamic constraints. To this end, we define a translation of metric formulas into monadic first-order formulas and give a correspondence between their models in Metric Equilibrium Logic and Monadic Quantified Equilibrium Logic, respectively. Interestingly, our translation provides a blue print for implementation in terms of ASP modulo difference constraints.

==> bbl.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}
\renewcommand{\url}[1]{\ignorespaces}
\renewcommand{\doi}[1]{\ignorespaces}

\bibitem{agcadipevi13a}
  Aguado, F., Cabalar, P., Di{\'e}guez, M., P{\'e}rez, G., Vidal, C.:
  Temporal equilibrium logic: a survey.
  Journal of Applied Non-Classical Logics \textbf{23}(1-2), 2--24 (2013).
  \doi{10.1080/11663081.2013.798985}

\bibitem{lpnmr19}
  Balduccini, M., Lierler, Y., Woltran, S. (eds.):
  Proceedings of the Fifteenth International Conference on Logic Programming and Nonmonotonic Reasoning (LPNMR'19),
  % Lecture Notes in Artificial Intelligence, vol. 11481.
  Springer (2019)

\bibitem{baboge05a}
  Baselice, S., Bonatti, P., Gelfond, M.:
  Towards an integration of answer set and constraint solving.
  In: % Gabbrielli, M., Gupta, G. (eds.)
  Proceedings of the Twenty-first International Conference on Logic Programming (ICLP'05).
  % Lecture Notes in Computer Science, vol.~3668,
  pp. 52--66. Springer (2005)

\bibitem{bedaei18a}
  Beck, H., Dao{-}Tran, M., Eiter, T.:
  {LARS:} {A} logic-based framework for analytic reasoning over streams.
  Artificial Intelligence \textbf{261}, 16--70 (2018).
  \doi{10.1016/j.artint.2018.04.003}

\bibitem{bocadisc18a}
  Bosser, A., Cabalar, P., Di\'eguez, M., Schaub, T.:
  Introducing temporal stable models for linear dynamic logic.
  In: % Thielscher, M., Toni, F., Wolter, F.  (eds.)
  Proceedings of the Sixteenth International Conference on Principles of Knowledge Representation and Reasoning (KR'18).
  pp. 12--21. {AAAI} Press (2018)

\bibitem{brzoska93a}
  Brzoska, C.:
  Temporal logic programming with metric and past operators.
  In: % Fisher, M., Owens, R. (eds.)
  Proceedings of the Workshop on Executable Modal and Temporal Logics.
  % Lecture Notes in Computer Science, vol.~897,
  pp. 21--39.  Springer (1995)

\bibitem{cadilasc20a}
  Cabalar, P., Di\'eguez, M., Laferriere, F., Schaub, T.:
  Implementing dynamic answer set programming over finite traces.
  In: % {De Giacomo}, G., Catal{\'a}, A., Dilkina, B., Milano, M., Barro, S., Bugar{\'{\i}}n, A., Lang, J. (eds.)
  Proceedings of the Twenty-fourth European Conference on Artificial Intelligence (ECAI'20).
  pp. 656--663. {IOS} Press (2020).
  \doi{10.3233/FAIA200151}

\bibitem{cadisc19a}
  Cabalar, P., Di{\'e}guez, M., Schaub, T.:
  Towards dynamic answer set programming over finite traces.
  In: % Balduccini et~al.
  \cite{lpnmr19},
  pp.  148--162.
  \doi{10.1007/978-3-030-20528-7\_12}

\bibitem{cadiscsc20a}
  Cabalar, P., Di{\'e}guez, M., Schaub, T., Schuhmann, A.:
  Towards metric temporal answer set programming.
  Theory and Practice of Logic Programming \textbf{20}(5), 783--798 (2020)

\bibitem{cakamosc19a}
  Cabalar, P., Kaminski, R., Morkisch, P., Schaub, T.:
  telingo = {ASP} + Time.
  In: % Balduccini et~al.
  \cite{lpnmr19},
  pp. 256--269.
  \doi{10.1007/978-3-030-20528-7\_19}

\bibitem{cakascsc18a}
  Cabalar, P., Kaminski, R., Schaub, T., Schuhmann, A.:
  Temporal answer set programming on finite traces.
  Theory and Practice of Logic Programming \textbf{18}(3-4), 406--420 (2018).
  \doi{10.1017/S1471068418000297}

\bibitem{cadiscsc21a}
  Cabalar, P., Di{\'{e}}guez, M., Schaub, T., Schuhmann, A.:
  Metric temporal answer set programming over timed traces (Extended abstract).
  In:
  Stream Reasoning Workshop (2021)

\bibitem{gimupape21a}
  {De Giacomo}, G., Murano, A., Patrizi, F., Perelli, G.:
  Timed trace alignment with metric temporal logic over finite traces.
  In: % Bienvenu, M., Lakemeyer, G., Erdem, E. (eds.)
  Proceedings of the Eighteenth International Conference on Principles of Knowledge Representation and Reasoning (KR'22).
  pp.  227--236. {AAAI} Press (2020).
  \doi{10.24963/kr.2021/22}

\bibitem{TIMEHandbook}
  Fisher, M., Gabbay, D., Vila, L. (eds.):
  Handbook of Temporal Reasoning in Artificial Intelligence, % Foundations of Artificial Intelligence, vol.~1.
  Elsevier Science (2005)

\bibitem{gekakaosscwa16a}
  Gebser, M., Kaminski, R., Kaufmann, B., Ostrowski, M., Schaub, T., Wanko, P.:
  Theory solving made easy with clingo~5.
  In: % Carro, M., King, A. (eds.)
  Technical Communications of the Thirty-second International Conference on Logic Programming (ICLP'16).
  % OpenAccess Series in Informatics (OASIcs), vol.~52,
  pp. 2:1--2:15.
  OASIcs % Schloss Dagstuhl--Leibniz-Zentrum fuer Informatik
  (2016)

\bibitem{hatiko00a}
  Harel, D., Tiuryn, J., Kozen, D.:
  Dynamic Logic. MIT Press (2000).
  \doi{10.1145/568438.568456}

\bibitem{heyting30a}
  Heyting, A.:
  Die formalen {R}egeln der intuitionistischen {L}ogik.
  In:
  Sitzungsberichte der Preussischen Akademie der Wissenschaften,
  pp. 42--56.
  Deutsche Akademie der Wissenschaften zu Berlin (1930)

\bibitem{hoflak18a}
  Hofmann, T., Lakemeyer, G.:
  A logic for specifying metric temporal constraints for golog programs.
  In: % Steinbauer, G., Ferrein, A. (eds.)
  Proceedings of the Eleventh Workshop on Cognitive Robotics (CogRob'18). % vol.~2325,
  pp. 36--46.
  {CEUR} Workshop Proceedings (2019).
  \url{http://ceur-ws.org/Vol-2325}

\bibitem{kamp68a}
  Kamp, J.:
  Tense Logic and the Theory of Linear Order.
  Ph.D. thesis, University of California at Los Angeles (1968)

\bibitem{koymans90a}
  Koymans, R.:
  Specifying real-time properties with metric temporal logic.
  Real-Time Systems \textbf{2}(4), 255--299 (1990)

\bibitem{lifschitz99b}
  Lifschitz, V.:
  Answer set planning.
  In: % {de Schreye}, D. (ed.)
  Proceedings of the International Conference on Logic Programming (ICLP'99).
  pp. 23--37. MIT Press (1999)

\bibitem{luvalibemc16a}
  Luo, R., Valenzano, R., Li, Y., Beck, C., McIlraith, S.:
  Using metric temporal logic to specify scheduling problems.
  In: % Baral, C., Delgrande, J., Wolter, F. (eds.)
  Proceedings of the Fifteenth International Conference on Principles of Knowledge Representation and Reasoning (KR'16).
  pp. 581--584. {AAAI} Press (2016)

\bibitem{ouawor07a}
  Ouaknine, J., Worrell, J.:
  On the decidability and complexity of metric temporal logic over finite words.
  Logical Methods in Computer Science \textbf{3}(1) (2007)

\bibitem{pearce96a}
  Pearce, D.:
  A new logical characterisation of stable models and answer sets.
  In: % Dix, J., Pereira, L., Przymusinski, T. (eds.)
  Proceedings of the Sixth International Workshop on Non-Monotonic Extensions of Logic Programming (NMELP'96).
  % Lecture Notes in Computer Science, vol.~1216,
  pp. 57--70.  Springer (1997).
  \doi{10.1007/BFb0023801}

\bibitem{peaval08a}
  Pearce, D., Valverde, A.:
  Quantified equilibrium logic and foundations for answer set programs.
  In: % {Garcia de la Banda}, M., Pontelli, E. (eds.)
  Proceedings of the Twenty-fourth International Conference on Logic Programming (ICLP'08).
  % Lecture Notes in Computer Science, vol.~5366,
  pp.  546--560. Springer (2008).
  \doi{10.1007/978-3-540-89982-2\_46}

\bibitem{pnueli77a}
  Pnueli, A.:
  The temporal logic of programs.
  In:
  Proceedings of the Eight-teenth Symposium on Foundations of Computer Science (FOCS'77).
  pp. 46--57. {IEEE} Computer Society Press (1977).
  \doi{10.1109/SFCS.1977.32}

\bibitem{sobatu04a}
  Son, T., Baral, C., Tuan, L.:
  Adding time and intervals to procedural and hierarchical control specifications.
  In: % McGuinness, D., Ferguson, G. (eds.)
  Proceedings of the Nineteenth National Conference on Artificial Intelligence (AAAI'04).
  pp. 92--97. {AAAI} Press (2004).
  \url{http://www.aaai.org/Library/AAAI/2004/aaai04-015.php}

\bibitem{wagrkaka19a}
  Wa{\l}ega, P., {Cuenca Grau}, B., Kaminski, M., Kostylev, E.:
  {DatalogMTL}: Computational complexity and expressive power.
  In: % Kraus, S. (ed.)
  Proceedings of the Twenty-Eighth International Joint Conference on Artificial Intelligence (IJCAI'19).
  pp. 1886--1892. ijcai.org (2019)

\bibitem{wakagr19a}
  Wa{\l}ega, P., Kaminski, M., {Cuenca Grau}, B.:
  Reasoning over streaming data in metric temporal datalog.
  In: % {Van Hentenryck}, P., Zhou, Z. (eds.)
  Proceedings of the Thirty-third National Conference on Artificial Intelligence (AAAI'19).
  pp. 3092--3099. {AAAI} Press (2019)

\end{thebibliography}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> include/asp-macros/dtel.tex <==
\RequirePackage{bm}
\RequirePackage{textcomp}
\RequirePackage{upgreek}

\IfFileExists{outline.tex}{\input{outline}}{}

\newcommand{\next}{\text{\rm \raisebox{-.5pt}{\Large\textopenbullet}}}  % {{\ensuremath{\circ}}}
\newcommand{\previous}{\text{\rm \raisebox{-.5pt}{\Large\textbullet}}}  % {{\ensuremath{\bullet}}}
\newcommand{\wnext}{\ensuremath{\widehat{\next}}}
\newcommand{\wprevious}{\ensuremath{\widehat{\previous}}}
\newcommand{\alwaysF}{\ensuremath{\square}}
\newcommand{\alwaysP}{\ensuremath{\blacksquare}}
\newcommand{\eventuallyF}{\ensuremath{\Diamond}}
\newcommand{\eventuallyP}{\ensuremath{\blacklozenge}}
\IfFileExists{outline.tex}
        {\newcommand{\until}{\ensuremath{\mathbin{\mbox{\outline{$\bm{\mathsf{U}}$}}}}}}
        {\newcommand{\until}{\ensuremath{\mathbin{\bm{\mathsf{U}}}}}}
\IfFileExists{outline.tex}
        {\newcommand{\release}{\ensuremath{\mathbin{\mbox{\outline{$\bm{\mathsf{R}}$}}}}}}
        {\newcommand{\release}{\ensuremath{\mathbin{\bm{\mathsf{R}}}}}}
\IfFileExists{outline.tex}
        {\newcommand{\while}{\ensuremath{\mathbin{\mbox{\outline{$\bm{\mathsf{W}}$}}}}}}
        {\newcommand{\while}{\ensuremath{\mathbin{\bm{\mathsf{W}}}}}}
\newcommand{\since}{\ensuremath{\mathbin{\bm{\mathsf{S}}}}}
\newcommand{\trigger}{\ensuremath{\mathbin{\bm{\mathsf{T}}}}}
\IfFileExists{outline.tex}
        {\newcommand{\finally}{\ensuremath{\mbox{\outline{$\bm{\mathsf{F}}$}}}}}
        {\newcommand{\finally}{\ensuremath{\bm{\mathsf{F}}}}}
\newcommand{\initially}{\ensuremath{\bm{\mathsf{I}}}}

\newcommand{\stp}{\ensuremath{\uptau}}

\newcommand{\dalways}[1]{\ensuremath{[#1]\,}}                        % \DBox
\newcommand{\deventually}[1]{\ensuremath{\langle#1\rangle\,}}        % \DDia
\newcommand{\drel}[2]{\ensuremath{{\parallel}{#1}{\parallel}^{#2}}}  % \Rel

\newcommand{\intervc}[2]{\ensuremath{[#1..#2]}}
\newcommand{\intervo}[2]{\ensuremath{[#1..#2)}}
\newcommand{\ointerv}[2]{\ensuremath{(#1..#2]}}
\newcommand{\rangec}[3]{\ensuremath{#1 \in \intervc{#2}{#3}}}
\newcommand{\rangeo}[3]{\ensuremath{#1 \in \intervo{#2}{#3}}}
\newcommand{\orange}[3]{\ensuremath{#1 \in \ointerv{#2}{#3}}}


==> include/asp-macros/grounding.tex <==
\newcommand{\ground}[1]{\ensuremath{\mathit{ground}(#1)}}
\newcommand{\cground}[2]{\ensuremath{\mathit{ground}_{#2}(#1)}}

\newcommand{\vars}[1]{\mathit{vars}(#1)}
\newcommand{\match}[2]{\mathit{match}_{#2}(#1)}


==> include/asp-macros/listings.tex <==
% The language definitions below require the following packages:
%
%     \usepackage{courier}
%     \usepackage{xcolor}
%     \usepackage{relsize}
%
%     \input{listings}
%     \renewcommand{\Underscore}{\textscale{1}{\textunderscore}}
%
% Without extra packages I had to provide an alternative underscore definition
% to get decent looking underscores.
%
% As an alternative to courier, it is also possible to use the `lmodern`
% package.
%
%     \usepackage[T1]{fontenc}
%     \usepackage{lmodern}
%     \usepackage{xcolor}
%     \usepackage{relsize}
%
%     \input{listings}
%
% When the python or clingo language is given, tex code can be embedded
% escaping it in `#( ... #)`, which is treated like a comment in Python.
% Furthermore, for logic programs the character sequence is `%%` is not output.
% This can be used to add labels at the end of lines. For example, in a logic
% program one can write
%
%     H :- B.%%#( \label{lst:rule} #)
%
% to refer to the rule from the document without having to worry about changing
% line numbers when refactoring. The annotated program will still be runnable
% with clingo.

\providecommand{\Underscore}{\textunderscore}

\lstdefinelanguage{clingo}{%
  basicstyle=\ttfamily,%
  keywordstyle=[1]\bfseries,%
  keywordstyle=[2]\bfseries,%
  keywordstyle=[3]\bfseries,%
  showstringspaces=false,%
  literate={_}{\Underscore}1 {\%\%}{}0,%
  escapeinside={\#(}{\#)},%
  alsoletter={\#,\&},%
  keywords=[1]{not,from,import,def,if,else,elif,return,while,break,and,or,for,in,del,and,class,with,as,is,yield,async},%
  keywords=[2]{\#const,\#show,\#minimize,\#base,\#theory,\#count,\#external,\#program,\#script,\#end,\#heuristic,\#edge,\#project,\#show,\#sum},%
  keywords=[3]{&,&dom,&sum,&diff,&show},%
  morecomment=[l]{\#\ },%
  morecomment=[l]{\%\ },%
  morestring=[b]",%
  stringstyle={\itshape},%
  commentstyle={\color{darkgray}}%
}

\lstdefinelanguage{python}{%
  basicstyle=\ttfamily,%
  keywordstyle=[1]\bfseries,%
  showstringspaces=false,%
  literate={_}{\Underscore}{1},%
  escapeinside={\#(}{\#)},%
  alsoletter={\#,\&},%
  keywords=[1]{not,from,import,def,if,else,elif,return,while,break,and,or,for,in,del,and,class,with,as,is,yield,async},%
  morecomment=[l]{\#\ },%
  morestring=[b]",%
  stringstyle={\itshape},%
  commentstyle={\color{darkgray}}%
}



==> include/asp-macros/modules.tex <==
% - modules ----------------------------------------
\newcommand{\module}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\prog}[1]{\ensuremath{P(#1)}}
\newcommand{\inp}[1]{\ensuremath{I(#1)}}
\newcommand{\out}[1]{\ensuremath{O(#1)}}
\newcommand{\inst}[2]{\ensuremath{#1(#2)}}
% \newcommand{\exts}{\epsilon}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> include/asp-macros/nogoods.tex <==
\newcommand{\domain}[1]{\ensuremath{\mathit{dom}(#1)}}

\newcommand{\ass}{\ensuremath{A}}

\newcommand{\tlits}[1]{\ensuremath{{#1}^{\true}}}
\newcommand{\flits}[1]{\ensuremath{{#1}^{\false}}}
\newcommand{\prefix}[2]{\ensuremath{#1[#2]}}

\newcommand{\clno}[1]{\ensuremath{\delta(#1)}}
\newcommand{\ClNo}[1]{\ensuremath{\Delta(#1)}}
% \newcommand{\nocl}[1]{\ensuremath{\gamma(#1)}}
% \newcommand{\NoCl}[1]{\ensuremath{\Gamma(#1)}}

\newcommand{\CN}[1]{\ensuremath{\Delta_{#1}}}
\newcommand{\LN}[1]{\ensuremath{\Lambda_{#1}}}

\newcommand{\dl}[0]{\ensuremath{\mathit{dl}}}
\newcommand{\dlevel}[1]{\ensuremath{\mathit{dlevel}(#1)}}
\newcommand{\opp}[1]{\ensuremath{\overline{#1}}}

% \newcommand{\undef}[0]{\ensuremath{\circ}}
% \newcommand{\trdef}[0]{\ensuremath{\times}}
\newcommand{\scc}[1]{\ensuremath{\mathit{scc}(#1)}}
\newcommand{\source}[1]{\ensuremath{\mathit{source}(#1)}}


==> include/asp-macros/operators.tex <==

% - operators ------------------------------------------------------------------

\newcommand{\Top}[1]{\ensuremath{T_{#1}}}
\newcommand{\T}[2]{\Top{#1}#2}
\newcommand{\Topi}[2]{\Top{#2}^{#1}}
\newcommand{\Ti}[3]{\Topi{#1}{#2}#3}

% - semantic operators -----------------------------------------------------------

\newcommand{\SM}[1]{\ensuremath{\mathit{SM}(#1)}}


==> include/asp-macros/outline.tex <==
\RequirePackage{xcolor}
\makeatletter

%%% MALIPIVO's PDF SPECIAL TO CHANGE FONT OUTLINE THICKNESS/COLOR
% https://tex.stackexchange.com/questions/18472/tikz-halo-around-text/169549#169549
\input pdf-trans
\newbox\qbox
\def\usecolor#1{\csname\string\color@#1\endcsname\space}
\newcommand\bordercolor[1]{\colsplit{1}{#1}}
\newcommand\fillcolor[1]{\colsplit{0}{#1}}
\newcommand\outline[1]{\leavevmode%
  \def\maltext{#1}%
  \setbox\qbox=\hbox{\maltext}%
  \boxgs{Q q 2 Tr \thickness\space w \fillcol\space \bordercol\space}{}%
  \copy\qbox%
}
\makeatother
\newcommand\colsplit[2]{\colorlet{tmpcolor}{#2}\edef\tmp{\usecolor{tmpcolor}}%
  \def\tmpB{}\expandafter\colsplithelp\tmp\relax%
  \ifnum0=#1\relax\edef\fillcol{\tmpB}\else\edef\bordercol{\tmpC}\fi}
\def\colsplithelp#1#2 #3\relax{%
  \edef\tmpB{\tmpB#1#2 }%
  \ifnum `#1>`9\relax\def\tmpC{#3}\else\colsplithelp#3\relax\fi
}
\bordercolor{black}
\fillcolor{white}
\def\thickness{.3}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> include/asp-macros/semantics.tex <==
\newcommand{\true}{\ensuremath{\boldsymbol{T}}}
\newcommand{\false}{\ensuremath{\boldsymbol{F}}}

\newcommand{\Cn}[1]{\ensuremath{\mathit{Cn}(#1)}}
\newcommand{\reduct}[2]{\ensuremath{#1^{#2}}}

\newcommand{\Loops}[1]{\ensuremath{\mathit{Loop}(#1)}}

% - formulas ---------------------------------------------------------------------

\newcommand{\BF}[1]{\ensuremath{\mathit{BF}(#1)}}
\newcommand{\CF}[1]{\ensuremath{\mathit{CF}(#1)}}
\newcommand{\LF}[1]{\ensuremath{\mathit{LF}(#1)}}

\newcommand{\CFIF}[1]{\ensuremath{\overleftarrow{\mathit{CF}}(#1)}}
\newcommand{\CFFI}[1]{\ensuremath{\overrightarrow{\mathit{CF}}(#1)}}
\newcommand{\CFX}[1]{\ensuremath{\mathit{CF}^x(#1)}}

\newcommand{\ES}[2]{\ensuremath{\mathit{ES}_{\!#2}(#1)}}
\newcommand{\EB}[2]{\ensuremath{\mathit{EB}_{\!#2}(#1)}}
\newcommand{\LFS}[2]{\ensuremath{\mathit{LF}_{\!#2}(#1)}}


==> include/asp-macros/syntax.tex <==
\newcommand{\head}[1]{\ensuremath{\mathit{h}(#1)}} % {\ensuremath{\mathit{head}(#1)}}
\newcommand{\Head}[1]{\ensuremath{\mathit{H}(#1)}}
\newcommand{\body}[1]{\ensuremath{\mathit{B}(#1)}} % {\ensuremath{\mathit{body}(#1)}}

\newcommand{\atom}[1]{\ensuremath{\mathit{A}(#1)}} % {\ensuremath{\mathit{atom}(#1)}}

\newcommand{\poslits}[1]{\ensuremath{{#1}^+}}
\newcommand{\neglits}[1]{\ensuremath{{#1}^-}}

\newcommand{\pbody}[1]{\poslits{\body{#1}}}
\newcommand{\nbody}[1]{\neglits{\body{#1}}}

\newcommand{\atbody}[2]{\ensuremath{\mathit{B}_{#1}(#2)}} % {\ensuremath{\mathit{body}_{#1}(#2)}}


==> include/asp-macros/tableau.tex <==

\newcommand{\Tsigned}[1]{\ensuremath{\true{#1}}}\message{ *** RENAME, Tlit,Flit ?? *** }
\newcommand{\Fsigned}[1]{\ensuremath{\false{#1}}}

\newcommand{\TOP}[1]{\ensuremath{D_{#1}}}
\newcommand{\COP}[1]{\ensuremath{D^*_{#1}}}

\newcommand{\Proviso}[1]{\raisebox{-7pt}[0pt][0pt]{\ensuremath{(#1)}}}

\newcommand{\plit}[1]{\ensuremath{\boldsymbol{t}{#1}}}
\newcommand{\nlit}[1]{\ensuremath{\boldsymbol{f}{#1}}}


==> proofs/strict.tex <==
\begin{proofof}{Proposition~\eqref{prop:strict}}
\\
\(
\next_{\intervo{m}{n}} \varphi {} \equiv \bigvee_{i=m}^{n{-}1} \metric{\next}{i}{i} \varphi   
\qquad\text{where }
\metric{\next}{i}{i}\varphi \eqdef
\begin{cases}
    \bot  \text{ if } i=0 \\
    {\alwaysF}_{\intervo{1}{i}} \bot \wedge \metric{\eventuallyF}{i}{i}\varphi  \text{ otherwise}
\end{cases}    
\)\\
From left to right: 
\(\M,k \models \next_{\intervo{m}{n}} \varphi\)
if $\M,k{+}1 \models \varphi$ 
 and $\tmf(k{+}1)-\tmf(k) \in \intervco{m}{n}$
and, since we are assuming strict traces, 
$\tmf(k{+}1)-\tmf(k) >0$.
Then
\(
\M,k \models \metric{\next}{i}{i} \varphi
\) for some $i>0 \in \intervco{m}{n}$. 
Then, since $i>0$, $\M,k \models \bigvee_{i=max(1,m)}^{n{-}1} \metric{\next}{i}{i} \varphi$.
Since there are no further states between $k$ and (the next state) $i$ allowed, we can conclude that $\M,k \models \alwaysF_{\intervo{1}{i}} \bot$.
Furthermore, since at some state $i \in \intervco{m}{n}$ formula $\varphi$ has to hold, we can conclude that $\M,k \models \metric{\eventuallyF}{i}{i}\varphi$. 
Putting both conclusions together we arrive at $\M,k \models \bigvee_{i=m}^{n{-}1}({\alwaysF}_{\intervo{1}{i}} \bot \wedge \metric{\eventuallyF}{i}{i}\varphi)$.
Finally, since the case of $i=0$ is redundant under the assumption of strict cases anyway, we arrive at:
\[
\M,k \models \bigvee_{i=m}^{n{-}1} \metric{\next}{i}{i} \varphi   
\qquad\text{where }
\metric{\next}{i}{i}\varphi \eqdef
\begin{cases}
    \bot  \text{if } i=0 \\
    {\alwaysF}_{\intervo{1}{i}} \bot \wedge \metric{\eventuallyF}{i}{i}\varphi  \text{ otherwise}
\end{cases}    
\]

From right to left, if 
\(
\M,k \models \bigvee_{i=m}^{n{-}1} \metric{\next}{i}{i} \varphi   
\qquad\text{where }
\metric{\next}{i}{i}\varphi \eqdef
\begin{cases}
    \bot  \text{if } i=0 \\
    {\alwaysF}_{\intervo{1}{i}} \bot \wedge \metric{\eventuallyF}{i}{i}\varphi  \text{ otherwise}
\end{cases}    
\), then 
\(
\M,k \models \bigvee_{i=max(1,m)}^{n{-}1} \metric{\next}{i}{i} \varphi
\), 
since $\metric{\next}{0}{0}$ becomes false by definition.
If we know that there is no state between $k$ and $i$, we can conclude that $i$ has to be the next state and therefore
\(
    \M,k \models \bigvee_{i=max(1,m)}^{n{-}1} \metric{\next}{i}{i} \varphi    
\)
Then, by the existential nature of the big disjunction, we can conclude that
\(
\M,k \models \metric{\next}{i}{i} \varphi
\text{ for some } i>0 \in \intervco{m}{n}   
\).
Since this implies
\(
M,k{+}1 \models \varphi 
\text{ and }
\tmf(k{+}1)-\tmf(k) \in \intervco{m}{n}
\text{ and }
\tmf(k{+}1)-\tmf(k) >0    
\)
we finally arrive at
\(
\M,k \models \next_{\intervo{m}{n}} \varphi    
\).       
\end{proofof}    
